Learning Low-Latency Action Verification for Frozen Vision-Language-Action Models

Vision-language-action (VLA) models have made significant progress in general-purpose robotic manipulation. However, sampled action sequences can be ineffective, while evaluating alternatives with computationally expensive verifiers adds latency at each policy query. In this work, we propose HDH, a lightweight framework that uses hindsight from a frozen VLA's own deployments to improve action verification. The framework has three stages. First, we deploy the policy and collect its autonomous rollouts. We then train a compact action verifier to assign each action chunk a predicted task-success score. Finally, the frozen VLA generates action candidates, and the verifier selects the candidate with the highest score for execution. Across four LIBERO-10 tasks, HDH achieves an average success rate of 82.3\% and on three real-world manipulation tasks, HDH improves average success over the baseline policy by 22.6\%.

==> tables/simulation.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{LIBERO Results (Simulation).}
Task success (\%), unweighted macro success, and end-to-end query latency
for the same frozen policy across four LIBERO tasks.
}
\label{tab:simulation}
\small
\renewcommand{\arraystretch}{1.12}
\setlength{\tabcolsep}{3pt}

\begin{tabularx}{\textwidth}{
    @{}l
    *{4}{>{\centering\arraybackslash}X}
    c
    cc@{}
}
\toprule
Method
& Soup + Sauce into Basket
& Bowl into Drawer + Close
& Mug on Plate + Pudding to Right
& Soup + Cheese into Basket
& Macro (\%)
& \multicolumn{2}{c}{Time/query (ms)} \\
& & & & & & p50 & p95 \\
\midrule
Baseline
& $73.3{\pm}2.5$
& $96.0{\pm}0.0$
& $66.0{\pm}2.8$
& $80.0{\pm}4.3$
& 78.8 & 681 & 760 \\

Random
& $64.0{\pm}2.8$
& $95.3{\pm}0.9$
& $66.7{\pm}6.6$
& $84.0{\pm}4.9$
& 77.5 & 692 & 776 \\

GPT-5
& $73.3{\pm}0.0$
& $93.3{\pm}0.0$
& $73.3{\pm}0.0$
& $73.3{\pm}0.0$
& 78.3 & 27,674 & 46,911 \\

GPT-6
& $69.3{\pm}6.6$
& $96.7{\pm}0.9$
& $72.0{\pm}7.5$
& $84.7{\pm}2.5$
& 80.7 & 7,403 & 10,270 \\

HDM
& $70.0{\pm}3.3$
& $98.7{\pm}0.9$
& $66.7{\pm}8.4$
& $86.0{\pm}4.3$
& 80.3 & 716 & 799 \\

HDH (Ours)
& $\mathbf{76.7{\pm}2.5}$
& $97.3{\pm}2.5$
& $72.0{\pm}5.9$
& $83.3{\pm}5.0$
& $\mathbf{82.3}$
& 718 & 796 \\
\bottomrule
\end{tabularx}
\end{table*}
